HAT-P-47b AND HAT-P-48b: Two Low Density Sub-Saturn-Mass Transiting Planets on the Edge of the Period--Mass Desert

We report the discovery of two new transiting extrasolar planets orbiting moderately bright (V = 10.7 and 12.2 mag) F stars (masses of 1.39 Msun and 1.10 Msun, respectively). The planets have periods of P = 4.7322 d and 4.4087 d, and masses of 0.21 MJ and 0.17 MJ which are almost half-way between those of Neptune and Saturn. With radii of 1.31 RJ and 1.13 RJ, these very low density planets are the two lowest mass planets with radii in excess that of Jupiter. Comparing with other recent planet discoveries, we find that sub-Saturns (0.18MJ < Mp < 0.3MJ) and super-Neptunes (0.05MJ < Mp < 0.18MJ) exhibit a wide range of radii, and their radii exhibit a weaker correlation with irradiation than higher mass planets. The two planets are both suitable for measuring the Rossiter-McLaughlin effect and for atmospheric characterization. Measuring the former effect would allow an interesting test of the theory that star-planet tidal interactions are responsible for the tendency of close-in giant planets around convective envelope stars to be on low obliquity orbits. Both planets fall on the edge of the short period Neptunian desert in the semi-major axis-mass plane.

==> HTR212-002_phfu_tab_short.tex <==
$ 55557.57382 $ & $   0.00470 $ & $   0.00053 $ & $   9.53342 $ & $ i$\\
$ 55557.57467 $ & $   0.00503 $ & $   0.00053 $ & $   9.53342 $ & $ i$\\
$ 55557.57553 $ & $   0.00555 $ & $   0.00054 $ & $   9.53607 $ & $ i$\\
$ 55557.57639 $ & $   0.00541 $ & $   0.00051 $ & $   9.53445 $ & $ i$\\
$ 55557.57724 $ & $   0.00570 $ & $   0.00050 $ & $   9.53334 $ & $ i$\\
$ 55557.57810 $ & $   0.00465 $ & $   0.00049 $ & $   9.53297 $ & $ i$\\
$ 55557.57895 $ & $   0.00446 $ & $   0.00049 $ & $   9.53267 $ & $ i$\\
$ 55557.57979 $ & $   0.00314 $ & $   0.00049 $ & $   9.53163 $ & $ i$\\
$ 55557.58065 $ & $   0.00211 $ & $   0.00049 $ & $   9.53065 $ & $ i$\\
$ 55557.58148 $ & $   0.00207 $ & $   0.00049 $ & $   9.53096 $ & $ i$\\


==> HTR212-002_rvtable.tex <==
$ 1557.93452 $ & $   -30.59 $ & $     7.79 $ & $     2.88 $ & $    21.90 $ & $    0.142 $ & $   0.086 $ & Keck \\
$ 1584.81706 $ & \nodata      & \nodata      & $   -14.87 $ & $    16.53 $ & $    0.145 $ & $   0.767 $ & Keck \\
$ 1584.86677 $ & $    55.12 $ & $     6.30 $ & $    -6.73 $ & $    21.22 $ & $    0.144 $ & $   0.777 $ & Keck \\
$ 1611.80587 $ & $    16.32 $ & $     6.83 $ & $     4.59 $ & $    35.18 $ & $    0.146 $ & $   0.470 $ & Keck \\
$ 1634.73217 $ & $    18.92 $ & $     6.11 $ & $    26.23 $ & $    35.18 $ & $    0.145 $ & $   0.315 $ & Keck \\
$ 1780.10010 $ & $   -17.66 $ & $    16.40 $ & \nodata      & \nodata      & \nodata      & $   0.034 $ & Subaru \\
$ 1780.10439 $ & $    -4.03 $ & $    19.70 $ & \nodata      & \nodata      & \nodata      & $   0.034 $ & Subaru \\
$ 1781.10948 $ & $    14.07 $ & $    17.07 $ & \nodata      & \nodata      & \nodata      & $   0.247 $ & Subaru \\
$ 1781.11548 $ & $   -31.26 $ & $     9.77 $ & \nodata      & \nodata      & \nodata      & $   0.248 $ & Subaru \\
$ 1781.12325 $ & $   -14.12 $ & $    13.00 $ & \nodata      & \nodata      & \nodata      & $   0.250 $ & Subaru \\
$ 1782.08387 $ & $   -16.86 $ & $    13.77 $ & \nodata      & \nodata      & \nodata      & $   0.453 $ & Subaru \\
$ 1782.09162 $ & $    -8.30 $ & $    15.18 $ & \nodata      & \nodata      & \nodata      & $   0.454 $ & Subaru \\
$ 1782.09938 $ & $     6.14 $ & $    16.01 $ & \nodata      & \nodata      & \nodata      & $   0.456 $ & Subaru \\
$ 1783.12240 $ & $    19.51 $ & $     6.59 $ & $    11.42 $ & $    14.82 $ & $    0.144 $ & $   0.672 $ & Keck \\
$ 1783.13154 $ & $    21.88 $ & $    12.45 $ & \nodata      & \nodata      & \nodata      & $   0.674 $ & Subaru \\
$ 1790.12677 $ & $   -41.16 $ & $     5.91 $ & $    10.85 $ & $    10.75 $ & $    0.147 $ & $   0.152 $ & Keck \\
$ 1791.12635 $ & $   -37.32 $ & $     7.00 $ & $    -2.77 $ & $     8.06 $ & $    0.146 $ & $   0.364 $ & Keck \\
$ 1796.11735 $ & $   -35.04 $ & $     7.99 $ & $   -10.40 $ & $    13.96 $ & $    0.146 $ & $   0.418 $ & Keck \\
$ 1807.12575 $ & $    21.94 $ & $     7.18 $ & $    24.75 $ & $    34.07 $ & $    0.146 $ & $   0.745 $ & Keck \\
$ 1812.08066 $ & $     5.64 $ & $     5.37 $ & $   -12.56 $ & $     6.83 $ & $    0.146 $ & $   0.792 $ & Keck \\
$ 1815.03365 $ & $   -23.62 $ & $     5.93 $ & $   -18.32 $ & $    10.50 $ & $    0.147 $ & $   0.416 $ & Keck \\
$ 1853.83582 $ & $    -2.77 $ & $     7.24 $ & $    19.24 $ & $    10.87 $ & $    0.144 $ & $   0.615 $ & Keck \\
$ 1870.96307 $ & $   -48.27 $ & $     6.35 $ & $     4.26 $ & $    10.85 $ & $    0.137 $ & $   0.235 $ & Keck \\
$ 1878.88618 $ & $     7.84 $ & $     6.01 $ & $    18.88 $ & $    14.82 $ & $    0.142 $ & $   0.909 $ & Keck \\
$ 1879.88871 $ & $     9.83 $ & $     6.88 $ & $    32.28 $ & $    14.30 $ & $    0.141 $ & $   0.121 $ & Keck \\
$ 1880.98816 $ & $    14.96 $ & $     5.95 $ & $    19.38 $ & $    11.22 $ & $    0.144 $ & $   0.353 $ & Keck \\
$ 1882.07816 $ & $    43.69 $ & $    10.01 $ & $   -42.58 $ & $    18.76 $ & $    0.133 $ & $   0.583 $ & Keck \\
$ 1944.76249 $ & $     4.30 $ & $     6.31 $ & $    -9.98 $ & $    11.80 $ & $    0.144 $ & $   0.830 $ & Keck \\
$ 1960.83339 $ & $   -10.87 $ & $     6.86 $ & $   -15.44 $ & $    17.99 $ & $    0.139 $ & $   0.226 $ & Keck \\
$ 1972.82552 $ & $    28.68 $ & $     4.82 $ & $     6.52 $ & $    11.75 $ & $    0.139 $ & $   0.760 $ & Keck \\
$ 1996.77476 $ & $   -34.83 $ & $    13.60 $ & $    -1.69 $ & $    31.67 $ & $    0.121 $ & $   0.821 $ & Keck \\
$ 2138.06092 $ & $    18.43 $ & $     7.48 $ & \nodata      & \nodata      & $    0.146 $ & $   0.678 $ & Keck \\


==> HTR213-008_phfu_tab_short.tex <==
$ 55574.58102 $ & $   0.00063 $ & $   0.00125 $ & $  10.95120 $ & $ i$\\
$ 55574.58164 $ & $  -0.00182 $ & $   0.00123 $ & $  10.94760 $ & $ i$\\
$ 55574.58244 $ & $  -0.00110 $ & $   0.00123 $ & $  10.95170 $ & $ i$\\
$ 55574.58307 $ & $   0.00250 $ & $   0.00122 $ & $  10.95370 $ & $ i$\\
$ 55574.58386 $ & $  -0.00287 $ & $   0.00122 $ & $  10.94890 $ & $ i$\\
$ 55574.58447 $ & $  -0.00085 $ & $   0.00121 $ & $  10.95090 $ & $ i$\\
$ 55574.58529 $ & $  -0.00063 $ & $   0.00122 $ & $  10.95050 $ & $ i$\\
$ 55574.58590 $ & $  -0.00006 $ & $   0.00122 $ & $  10.95010 $ & $ i$\\
$ 55574.58671 $ & $  -0.00339 $ & $   0.00122 $ & $  10.94660 $ & $ i$\\
$ 55574.58733 $ & $  -0.00118 $ & $   0.00122 $ & $  10.94970 $ & $ i$\\


==> HTR213-008_rvtable.tex <==
$ 1557.94958 $ & $   -37.91 $ & $     5.66 $ & $   -31.23 $ & $    11.12 $ & $    0.122 $ & $   0.203 $ & Keck \\
$ 1584.83402 $ & \nodata      & \nodata      & $    15.76 $ & $     9.32 $ & $    0.135 $ & $   0.301 $ & Keck \\
$ 1584.85683 $ & $   -18.72 $ & $     4.16 $ & $   -19.17 $ & $    24.21 $ & $    0.137 $ & $   0.306 $ & Keck \\
$ 1611.83497 $ & $    -4.56 $ & $     5.27 $ & $    46.93 $ & $    12.76 $ & $    0.126 $ & $   0.425 $ & Keck \\
$ 1634.74237 $ & $    43.01 $ & $     4.92 $ & $    15.71 $ & $    32.57 $ & $    0.141 $ & $   0.621 $ & Keck \\
$ 1779.68487 $ & $    21.90 $ & $     9.20 $ & \nodata      & \nodata      & \nodata      & $   0.498 $ & FIES \\
$ 1780.07705 $ & $    16.14 $ & $     9.54 $ & $    -9.11 $ & $    23.26 $ & \nodata      & $   0.587 $ & Subaru \\
$ 1780.08485 $ & $    14.42 $ & $     8.61 $ & $     6.75 $ & $    21.41 $ & \nodata      & $   0.589 $ & Subaru \\
$ 1780.09261 $ & $    -4.77 $ & $    10.40 $ & $    10.18 $ & $    21.93 $ & \nodata      & $   0.591 $ & Subaru \\
$ 1780.70889 $ & $    11.50 $ & $     9.40 $ & \nodata      & \nodata      & \nodata      & $   0.730 $ & FIES \\
$ 1781.05224 $ & $    22.34 $ & $     9.27 $ & $    -3.01 $ & $    22.96 $ & \nodata      & $   0.808 $ & Subaru \\
$ 1781.06001 $ & $    28.26 $ & $     7.48 $ & $     5.59 $ & $    22.00 $ & \nodata      & $   0.810 $ & Subaru \\
$ 1781.06778 $ & $    15.23 $ & $     7.31 $ & $     7.32 $ & $    21.53 $ & \nodata      & $   0.812 $ & Subaru \\
$ 1781.08022 $ & \nodata      & \nodata      & $    -2.25 $ & $    21.00 $ & \nodata      & $   0.815 $ & Subaru \\
$ 1781.09494 $ & \nodata      & \nodata      & $     6.19 $ & $    26.40 $ & \nodata      & $   0.818 $ & Subaru \\
$ 1781.69965 $ & $   -11.80 $ & $     8.00 $ & \nodata      & \nodata      & \nodata      & $   0.955 $ & FIES \\
$ 1782.05225 $ & $   -18.74 $ & $    12.80 $ & $     4.20 $ & $    23.72 $ & \nodata      & $   0.035 $ & Subaru \\
$ 1782.06002 $ & $     0.11 $ & $    10.76 $ & $   -14.68 $ & $    24.22 $ & \nodata      & $   0.037 $ & Subaru \\
$ 1782.07119 $ & $   -13.29 $ & $     7.84 $ & $     4.39 $ & $    24.52 $ & \nodata      & $   0.039 $ & Subaru \\
$ 1783.09288 $ & $   -20.51 $ & $    11.55 $ & $     0.85 $ & $    23.79 $ & \nodata      & $   0.271 $ & Subaru \\
$ 1783.10066 $ & $    -9.15 $ & $     8.94 $ & $   -11.30 $ & $    24.06 $ & \nodata      & $   0.273 $ & Subaru \\
$ 1783.11016 $ & $   -10.90 $ & $     8.80 $ & $     0.01 $ & $    20.35 $ & \nodata      & $   0.275 $ & Subaru \\
$ 1815.04453 $ & $   -24.25 $ & $     4.12 $ & $   -20.78 $ & $     8.20 $ & $    0.145 $ & $   0.519 $ & Keck \\
$ 1853.84571 $ & $    -3.11 $ & $     4.22 $ & $    32.51 $ & $     9.70 $ & $    0.136 $ & $   0.320 $ & Keck \\
$ 1857.57640 $ & $   -29.20 $ & $    12.30 $ & \nodata      & \nodata      & \nodata      & $   0.166 $ & FIES \\
$ 1858.63379 $ & $    15.50 $ & $    12.10 $ & \nodata      & \nodata      & \nodata      & $   0.406 $ & FIES \\
$ 1859.65351 $ & $     6.90 $ & $     8.00 $ & \nodata      & \nodata      & \nodata      & $   0.637 $ & FIES \\
$ 1877.94245 $ & $    37.27 $ & $     4.28 $ & $  -100.83 $ & $    36.09 $ & $    0.139 $ & $   0.785 $ & Keck \\
$ 1882.10175 $ & $    -8.16 $ & $     4.99 $ & $  -131.16 $ & $    58.69 $ & $    0.122 $ & $   0.729 $ & Keck \\
$ 1944.81352 $ & $    12.26 $ & $     4.61 $ & $   -10.28 $ & $     9.25 $ & $    0.136 $ & $   0.954 $ & Keck \\
$ 1964.77835 $ & $   -14.35 $ & $     8.57 $ & $     4.29 $ & $    22.52 $ & \nodata      & $   0.482 $ & Subaru \\
$ 1964.78611 $ & $    -4.14 $ & $     9.71 $ & $   -12.71 $ & $    24.55 $ & \nodata      & $   0.484 $ & Subaru \\
$ 1964.79387 $ & $     3.39 $ & $     9.95 $ & $   -16.91 $ & $    21.30 $ & \nodata      & $   0.486 $ & Subaru \\
$ 1967.81621 $ & $    -8.31 $ & $    11.72 $ & $    -1.74 $ & $    25.87 $ & \nodata      & $   0.171 $ & Subaru \\
$ 1967.83092 $ & $   -21.10 $ & $    10.71 $ & $    10.02 $ & $    19.76 $ & \nodata      & $   0.175 $ & Subaru \\
$ 1967.84563 $ & $   -28.85 $ & $    11.18 $ & $    11.92 $ & $    24.22 $ & \nodata      & $   0.178 $ & Subaru \\


==> Makefile <==
TARGET=hatpxx
PRINTER=cfa_ssplw

all: $(TARGET).pdf

SUB=submit_v1

.PHONY: all clean save print

$(TARGET).dvi: *.tex *.cls
	latex $(TARGET).tex
	bibtex $(TARGET)
	latex $(TARGET).tex
	latex $(TARGET).tex

$(TARGET).ps: $(TARGET).dvi
	dvips -t letter $(TARGET).dvi -o

$(TARGET).pdf: $(TARGET).ps
	ps2pdf $< $@

save:
	tar cvf $(TARGET).tar *
	gzip $(TARGET).tar
	mv $(TARGET).tar.gz $(TARGET).tgz

clean:
	rm -f *.ps *.dvi *.aux *.log *.pdf \
        $(TARGET).idx $(TARGET).inx $(TARGET).toc $(TARGET).tgz \
        $(TARGET)Notes.bib

print: $(TARGET).ps
	lpr -P$(PRINTER) $<

